Optimization of the Multigrid-Convergence Rate on Semi-structured Meshes by Local Fourier Analysis

In this paper a local Fourier analysis for multigrid methods on tetrahedral grids is presented. Different smoothers for the discretization of the Laplace operator by linear finite elements on such grids are analyzed. A four-color smoother is presented as an efficient choice for regular tetrahedral grids, whereas line and plane relaxations are needed for poorly shaped tetrahedra. A novel partitioning of the Fourier space is proposed to analyze the four-color smoother. Numerical test calculations validate the theoretical predictions. A multigrid method is constructed in a block-wise form, by using different smoothers and different numbers of pre- and post-smoothing steps in each tetrahedron of the coarsest grid of the domain. Some numerical experiments are presented to illustrate the efficiency of this multigrid algorithm.

==> hhg.tex <==
For solving elliptic PDEs, FE methods are often preferred over other
discretization schemes, because they permit flexible, unstructured
meshes. Among the MG methods, algebraic MG \cite{Yang:2006:LNCSE} also supports
unstructured meshes automatically. Geometric MG, in contrast, relies on a given
hierarchy of nested meshes. On the other hand, geometric MG achieves a
significantly higher performance than algebraic MG in terms of unknowns
computed per second.

The Hierarchical Hybrid Grids (HHG) software framework
\cite{Bergen:2006:CiSE,Bergen:2005:SC05} is designed to close this gap between
FE flexibility and geometric MG performance by using a compromise between
structured and unstructured grids. A coarse input FE mesh is organized into the
grid primitives vertices, edges, faces, and volumes. The primitives are then
refined in a structured way, as indicated in Figure \ref{fig:2d_levels}.

\begin{figure}
  \caption{\label{fig:2d_levels} Regular refinement example for a
    two-dimensional input mesh. Beginning with the input mesh on the left, each
    successive level of refinement creates a new mesh that has a larger number
    of interior points with structured couplings.}

  %\vspace*{1.0ex}
  \centering
  \includegraphics[width=\textwidth]{figures/2d_levels_series.pdf}
\end{figure}

The HHG data layout preserves the flexibility of unstructured meshes, while the
regular internal structure of the primitives allows for an efficient
implementation on current computer architectures, especially on parallel
computers. In parallel runs on up to 16\,384 cores HHG has demonstrated
excellent performance on solving linear systems with up to $3 \cdot 10^{11}$
unknowns. The semi-structured mesh also subserves the local adaption of the
smoothing parameters needed in \Sec{sec:localadapt}.




==> smoothers.tex <==
In a multigrid algorithm, the smoother has the task of reducing the
high-frequent error components, while the coarse grid correction reduces the
low-frequents components. Both smoother and coarse grid correction can be tuned
to optimally suit the numerical problem, \ie{} the differential equation and
its discretization. In this paper, we focus on optimizing the smoother for
anisotropic discretizations. We compare the widely used Jacobi and Gauss-Seidel
smoothers to a four-color smoother and a line smoother. Besides choosing the
smoother type, two more parameters can be changed to achieve optimal smoothing
results: the under-/over-relaxation parameter $\omega$ and the number of
pre-/post-smoothing steps per multigrid cycle $\nu_1$ and $\nu_2$. These
parameters can even be adapted locally, if the numerical properties change
strongly across the domain. Implementing local adaptivity can be quite easy and
very effective, as \Sec{sec:results} will show. The remainder of this section
introduces the investigated smoothers.

In the \emph{Jacobi} algorithm, all updated values only depend on values from
the previous iteration. On the one hand, this allows for excellent
parallelization, on the other hand, it requires more memory to keep all values
from the previous iteration. In a straight-forward implementation, the storage
for two times the number of unknowns is required. The Jacobi algorithm is fast,
but it has a bad convergence rate.

In a \emph{Gauss-Seidel} iteration, values that have already been updated in
the current iteration are used in the same iteration for updating dependent
values. Thus, the unknowns have to be stored only once. If the grid points are
updated in a \emph{lexicographical order}, a grid point update depends on data
from the directly preceding update. This data dependency inhibits a
straight-forward parallelization.

The Gauss-Seidel algorithm usually smoothes much better than the Jacobi
algorithm, but, due to its data dependencies, it is potentially much slower on
current hardware. The data dependencies can be eliminated by grouping the grid
points into ``colors''. Points of the same color are not connected to each
other, so they can be updated in parallel. The discretization determines the
required number of colors. In a 2D rectangular grid with a 5-point
discretization stencil, for example, two colors are needed (\cf{}
\Fig{fig:coloring_5point}). The 15-point stencil of HHG needs \emph{four
  colors} (\cf{} \Fig{fig:coloring_15point}). Note that the relaxation
parameter $\omega$ can be set individually for each of the colors.

\begin{figure}
  \begin{minipage}[t]{1.0\textwidth}
%    \setlength{\figcaptionwidth}{\textwidth}%
    \caption {\label{fig:coloring}Stencil colorings.}
    \subfigure[][\label{fig:coloring_5point}Coloring of a 5-point stencil.]{\hspace*{0.5\textwidth}}\hfill%
    \subfigure[][\label{fig:coloring_15point}Coloring of a 15-point stencil.]{\hspace*{0.5\textwidth}}
  \end{minipage}\vspace{-3ex}\\\vspace{-3ex}%
  \begin{minipage}{0.5\textwidth}
    \centering%
    \includegraphics[scale=0.33]{stencil_5point.pdf}%
  \end{minipage}\hfill%
  \begin{minipage}{0.5\textwidth}
    \centering%
   \includegraphics[scale=0.33]{stencil_15point_4color_e.pdf}%
  \end{minipage}%
\end{figure}

\begin{figure}[htb]
\centering{\includegraphics[height=6cm,width=7cm]{stencil_15point_4color_e.pdf}}
\caption{Polygonal domain of the convection-diffusion problem and the grid after twice refinement process.}
\label{dominio3}
\end{figure}
Instead of updating single unknowns like in the previous cases, we can also
update a \emph{line of unknowns} at a time. Therefore, we have to solve a
tridiagonal system of equations. This can be achieved either by repeated
smoothing or by using a direct solver, like a modified Gauss elimination,
applied to the line. While the lines can be updated in different orders, we
will restrict ourselves to the lexicographic ordering in the remainder of this
paper.

